Capacity-Approaching Autoencoders for Communications

The autoencoder concept has fostered the reinterpretation and the design of modern communication systems. It consists of an encoder, a channel, and a decoder block which modify their internal neural structure in an end-to-end learning fashion. However, the current approach to train an autoencoder relies on the use of the cross-entropy loss function. This approach can be prone to overfitting issues and often fails to learn an optimal system and signal representation (code). In addition, less is known about the autoencoder ability to design channel capacity-approaching codes, i.e., codes that maximize the input-output information under a certain power constraint. The task being even more formidable for an unknown channel for which the capacity is unknown and therefore it has to be learnt. In this paper, we address the challenge of designing capacity-approaching codes by incorporating the presence of the communication channel into a novel loss function for the autoencoder training. In particular, we exploit the mutual information between the transmitted and received signals as a regularization term in the cross-entropy loss function, with the aim of controlling the amount of information stored. By jointly maximizing the mutual information and minimizing the cross-entropy, we propose a methodology that a) computes an estimate of the channel capacity and b) constructs an optimal coded signal approaching it. Several simulation results offer evidence of the potentiality of the proposed method.

==> Architecture.tex <==
\section{Architecture}

==> Biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/IEEE_Alex}}]{Nunzio A. Letizia} received the Laurea Magistrale degree in electrical engineering (summa cum laude) in 2018 from the University of Udine, Italy. During his studies he was awarded with a full scholarship at Scuola Superiore dell'Universit\'a degli studi di Udine. His research interests spread from mathematics and
physics to communication engineering. He is working towards the Ph.D. at the University of Klagenfurt, Austria. His research areas are signal processing and statistical learning.
\end{IEEEbiography}
\vskip 0pt plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pics/prof1}}]{Andrea M. Tonello}
received the D.Eng. degree (Hons.) in electronics and the D.Res. degree in electronics and telecommunications from the University of Padova, Italy, in 1996 and 2002, respectively. From 1997 to 2002, he was with Bell Labs-Lucent Technologies, Whippany, NJ, USA, as a member of the Technical Staff. Then, he was promoted to Technical Manager and appointed to Managing Director of the Bell Labs Italy Division. In 2003, he joined the University of Udine, Udine, Italy, where he became an Aggregate Professor in 2005 and an Associate Professor in 2014. He is currently Professor of Embedded Communication Systems at the University of Klagenfurt, Klagenfurt, Austria. He is also the Founder of the spinoff company, WiTiKee. He received several awards, including the Distinguished Visiting Fellowship from the Royal Academy of Engineering, U.K. (2010), the IEEE VTS and COMSOC Distinguished Lecturer Awards (2011, 2015, 2018), the UC3M Chair of Excellence (2019-2020) and nine best paper awards. He served/s as an Associate Editor of the IEEE Trans. on Vehicular Techn., IEEE Trans. on Communications, IEEE Access, and IET Smart Grid. He has been appointed Director of Industry Outreach of the IEEE ComSoc for the term 2020-2021.
\end{IEEEbiography}


==> Related_Work.tex <==
\section{Background}
\label{sec:Related_Work}







